Nucleon Scalar and Tensor Charges from Lattice QCD with Light Wilson Quarks

We present 2+1 flavor Lattice QCD calculations of the nucleon scalar and tensor charges. Using the BMW clover-improved Wilson action with pion masses between 150 and 350 MeV and three source-sink separations between 0.9 and 1.4 fm, we achieve good control over excited-state contamination and extrapolation to the physical pion mass. As a consistency check, we also present results from calculations using unitary domain wall fermions with pion masses between 300 and 400 MeV, and using domain wall valence quarks and staggered sea quarks with pion masses between 300 and 600 MeV.

==> Makefile <==
all-tex		= paper.tex
all-bib		= paper.bib

text-dir	= text
figs-dir	= figs


ps-figs		= \


eps-figs	= \


pdf-figs	= \


include make.tex.inc

